Warp and Learn: Novel Views Generation for Vehicles and Other Objects

In this work we introduce a new self-supervised, semi-parametric approach for synthesizing novel views of a vehicle starting from a single monocular image. Differently from parametric (i.e. entirely learning-based) methods, we show how a-priori geometric knowledge about the object and the 3D world can be successfully integrated into a deep learning based image generation framework. As this geometric component is not learnt, we call our approach semi-parametric. In particular, we exploit man-made object symmetry and piece-wise planarity to integrate rich a-priori visual information into the novel viewpoint synthesis process. An Image Completion Network (ICN) is then trained to generate a realistic image starting from this geometric guidance. This careful blend between parametric and non-parametric components allows us to i) operate in a real-world scenario, ii) preserve high-frequency visual information such as textures, iii) handle truly arbitrary 3D roto-translations of the input and iv) perform shape transfer to completely different 3D models. Eventually, we show that our approach can be easily complemented with synthetic data and extended to other rigid objects with completely different topology, even in presence of concave structures and holes (e.g. chairs). A comprehensive experimental analysis against state-of-the-art competitors shows the efficacy of our method both from a quantitative and a perceptive point of view. Supplementary material, animated results, code and data are available at: https://github.com/ndrplz/semiparametric

==> figures/appearance_transfer.tex <==
\begin{figure*}[bh]
    \centering
    \includegraphics[width=0.98\textwidth]{images/car_shape_transfer.pdf}
    \caption{Appearance transfer to different 3D models; it can be appreciated how the network performs a reasonable transfer of object's appearance even when the destination 3D model is highly different to the input one.}
    \label{fig:app_transfer}
\end{figure*}
% \begin{figure}[b]
%     \centering
%     \includegraphics[width=0.95\columnwidth]{images/app_transfer.png}
%     \caption{Appearance transfer to different 3D models; it can be appreciated how the network performs a reasonable transfer of object's appearance even when the destination 3D model is highly different to the input one.}
%     \label{fig:app_transfer}
% \end{figure}

==> figures/suppl_pascal_aug.tex <==
\begin{figure}[tbh]
    \centering
    \includegraphics[width=0.95\columnwidth]{images/suppl_pascal_aug.pdf}
    \caption{Examples of additional data generated stitching generated vehicles onto \pascal backgrounds.}
    \label{fig:suppl:pascal_aug}
\end{figure}

==> figures/vis_model.tex <==
\begin{figure}[th]
    \centering
    \includegraphics[width=0.99\columnwidth]{images/vis_model.pdf}
    \caption{Scheme of the patch visibility model. Details in Sec.~\ref{subsec:visibility}.}
    \label{fig:vis_model}
\end{figure}

==> rebuttal_iccv/figures/rotation_chair.tex <==
\begin{figure}[th]
    \centering
    \includegraphics[width=0.98\columnwidth]{images/rotation_chair.pdf}
    \caption{Results of 360° rotation for chairs. Zoom for details.}
    \label{fig:rebut:rotation_chair}
\end{figure}

==> rebuttal_iccv/tables/table_fid.tex <==
\begin{table}[b]
\begin{center}
\setlength\tabcolsep{6pt} % reduce space between cols
\begin{tabular}{l|cccccc}
    \toprule
    & ours & \cite{zhu2018visual} & \cite{esser2018variational} & \cite{tatarchenko2016multi} & \cite{park2017transformation} & \cite{sun2018multi}\\
    \midrule
\textit{car} & 43.1 & 86.4 & 72.4 & 269.6 & 80.3 & 159.6\\
\textit{chair} & 58.3 & 82.2 & 73.5 & - & 90.8 & 181.9\\
\bottomrule
\end{tabular}
\end{center}
\caption{\fids results on \pascal.}
\label{tab:rebut:fid}
\end{table}

==> rebuttal_tpami/r1.tex <==
\Large{{\bf R1}}\normalsize
\\\\

\response
{
    p2 ln 51-52: "these approaches are limited by the need to be trained solely on synthetic data". This does not seem to be the case. One can imagine a *real* dataset of object videos with SfM-annotated cameras, which can then be used to supervise a new-view synthesis pipeline.
}
{
    We agree with R1 that in principle an extensive campaign of data collection could lead to such a dataset. We have rephrased the sentence to reflect this. However, we argue that appropriately covering the intra-variance of each class for a significant number of classes is extremely challenging, costly and time-consuming. This is even more true when training deep networks, which are notoriously sample-inefficient and require massive amount of diverse training data, leading most methods to rely on synthetic datasets in practice.
}

\response
{
    p3 ln 16-17: The list of recent methods ends with works from CVPR 2018. I think authors should also add recent papers from ICCV19, NeurIPS19 on this topic.
}
{
    The related works section has been extended to include recent works from the scientific community which were published after our submission in October 2019.
}

\response
{
    Sec 3.1: Why are the 2D keypoints needed at all? Wouldn't it be possible to generate the ground truth warps using the knowledge of the relative viewpoint and the depth of the rendered part of the CAD model?
}
{
    We use 2D keypoints to describe class-dependent planes which are sliced from the source image and fed to the network through dedicated channels in the input tensor.
    We agree that in principle one could get those 2D keypoints by projecting the 3D keypoints of the CAD model. However there are two main challenges:
    \begin{itemize}
        \item \pascal is very coarsely annotated with regards to the CAD models (e.g. only a few different models cover the whole vehicle class). Even with a perfect alignment between the CAD and the source image, the mismatch between the 3D model and the actual car in the image would cause a misalignment for the planes;
        \item At inference time, it's easier to get a reasonably aligned viewpoint using 2D keypoints and 3D CAD information (e.g. through PnP matching) than the other way around.
    \end{itemize}
     On the other hand, the depth information could be used to determine a number of visible planes (using for example a RANSAC-based approach) or to warp individual pixels. We will consider these approaches as future works.  
}

\response
{
    Sec 3.5: The fact that authors provide only a tiny center crop seems sub-optimal. Why not adding the whole crop? The central crop (probably) does not contain details on the borders of the car such as the color of the lights or the style of the wheels.
}
{
    The goal of the center crop is not to provide detailed information to the network, but only give a hint about the average color of the object (i.e. an appearance prior). We also experimented providing the full crop to the network, but this resulted in poor results on validation set, despite a very low self-supervised loss during training.
    Since we optimize the reconstruction error with respect to the input image, the network learns to simply forward the appearance prior information directly to the output layer. 
}

\response
{
    Pascal3D contains 12 categories and only 2 are evaluated. While I recognize the effort it takes to make all the baselines work on all categories, it would be great to at least see qualitative results of the proposed method on as many categories as possible. Can authors provide qualitative eval for say 5 more categories with the largest number of annotations?
}
{
    When designing this work, vehicles have always been the main class of interest. We decided to add the chair class because most of competitors benchmark on this couple (car $+$ chair). 
    However, we understand the legitimate concern about the generality of the method, so we include qualitative results for other 3 classes from \pascal dataset in Sec.7 of the supplementary material.
    It's worth noticing that some of the \pascal classes are not suitable for evaluation due to either non-planarity (e.g. \textit{bottle}) or non-fixed number of keypoints (e.g. \textit{boat}, \textit{table}). Also, all these classes have way less images than the car and chair classes.
    Results show that our framework is able to handle a diverse set of object classes, provided that the underlying constraints (i.e. object symmetry, piece-wise planarity) hold.
}

\response
{
    Table 2: Here I am not sure why did authors omit comparison to TVSN which is quite clearly the most comparable baseline? 
}
{
    When designing the A/B perceptual experiments we decided to include only methods that could be trained on real data (i.e. \pascal) to ensure fairness. Looking back on this choice, we acknowledge a wider range of competitors could have been included in the evaluation. However, repeating the experiments including all 6 comparison is extremely expensive and time consuming and we couldn't manage to squeeze it in the short rebuttal phase.
}

\response
{
    Table 2: it seems that fine-tuning of VON actually makes its results worse?
}
{
    We noticed that results from VON exhibit a noticeable variance in terms of quality across different viewpoints (see Fig.~1 from the supplementary materials). We suspect that fine-tuning it on Pascal+ had further strengthened this variance, as most of the training pictures comes from lateral viewpoints. In fact, while for some viewpoints results improve, others see a noticeable drop in performance.
}

\response
{
    Table 1: Can authors provide an intuition on why there is a large increase in error for 180/0 degrees relative viewpoint difference? Please make the best result in each column bold to facilitate visual ranking of the results.
}
{
    Front and rear views are less common in the \pascal dataset, which makes predictions around those angles particularly challenging.
    In this case our method often operates into an almost complete absence of prior information, as lateral planes are likely dropped during the transformation (e.g. when going from left to front side view, the side is not visible anymore in the destination viewpoint). This results in a texture-less shape inferred from the 2.5D sketch and a higher \fid.
    
    Also learning-based approaches like VON or TVSN fail more frequently for those viewpoint. However, we observed that the most common failure mode is the generation of a blob-like shape filled with textures from the source image. Even though this is extremely unrealistic for the human eye it's rewarded by the \fid as it preserves textures.
}

\response
{
    Fig. 5: Please provide qualitative results of the ablation study as well.
}
{
    We are not sure about what R1 means. Fig.~5 is indeed the qualitative overview of the ablation results.
}

\response
{
    p8 ln 30-32: "our method out performs all competitors" ... In fact, the proposed method is outperformed for some of the relative angles. While I agree that on average the method is indeed the best, I would expand the sentence to slightly soften the claim.
}
{
    We have softened our claim to better reflect the table's results.
}


==> rebuttal_tpami/r2.tex <==
\Large{{\bf R2}}\normalsize
\\\\

\response
{
    The paper uses ground truth key points for training the method and generating novel views. How would it perform on predicted keypoints in the wild ? This is important to demonstrate the robustness of the method for small errors in detected keypoints.
}
{
    Good point. We experimented adding isotropic Gaussian noise to the 2D keypoints locations to simulate a more real-world scenario. We included the discussion and a chart showing the results in a new section of the supplementary due to space limitations in the main paper. As a side note, our approach has been recently tested in a real-world scenario in a recent ICPR 2020 paper
    (\url{https://arxiv.org/pdf/2007.00323.pdf}).
}

\response
{
    The suggested method focuses on producing detailed textures rather than detailed geometry. It only works for objects with small number of planer surfaces and Not able to represent detailed geometry. This and other limitations needs to be discussed clearly in the paper.
}
{
    We agree that the main purpose of this work is producing detailed textures. Geometry is so to say built-in in the framework, it's not something we want to infer. In principle our method can also deal with complex geometry and large number of planes. Obviously that is challenging in practice, because this fine-grained data might not be readily available. On the contrary, working with a relatively small set of planes makes feasible to get the required geometry information (e.g. annotating / detecting the 2D keypoints). We stressed the constraints of our proposed method in multiple points where we mention that this method is designed only to deal with symmetric, man-made objects.
}

\response
{
    The method uses paired dataset for 3D objects and images ( AKA Pascal3D+) for training. This is a difficult data requirement and predicting the 3D shape or pose from the image can introduce additional robustness problems which is not discussed in the paper.
}
{
    We agree that having images with aligned 3D models is an expensive annotation. 
    We argue that the majority of our competitors either share the same requirements or directly train on synthetic data (e.g. ShapeNet).
    At test time, we can rely on a robust 2D keypoint detector and a coarse model classifier to estimate the viewpoint via PnP matching (please see also to the ICPR 2020 paper above \url{https://arxiv.org/pdf/2007.00323.pdf}).
}

\response
{
    Page 7 lines 54 - 57: Why is feeding the 2.5D sketch to VUNet is more informative than the original input of skeleton, edges or keypoints? This statement not clear.
}
{
   The original skeleton consists of a set of lines connecting the different keypoints of the object. We replaced this representation with the 2.D sketch, which also includes the direction of the normal surfaces and fine-grained details from the 3D model. We have rephrased the sentence to better reflect this point.
}

\response
{
    Request experiment with only using the appearance prior and the 2.5D sketch.
}
{
    We have run this additional experiment, but due to space limitations we include qualitative results in supplementary materials (Sec.9). In line with our expectation, when the network is not provided with any planes to warp during train the result is almost completely texture-less. Thanks to the appearance prior though, the average color is successfully applied to the final result.
}

\response
{
    The method only uses a small number of 3D object models which makes it questionable how well it can extend to other object classes with more variance in 3D shape.
}
{
    We don't consider the number of 3D models an intrinsic limitation of our model. In fact, because the process is guided by the 2.5 sketch, we expect it to cope well with variations in the shape. Clearly, this holds true as long as the variation still allows to detect a predefined set of keypoints.  
}

\response
{
    The self-supervised loss can be better described as adversarial loss
}
{
    Our training objective has indeed both a perceptual and an adversarial component. Regardless of what is under the hood, we refer to it as self-supervised to highlight the fact that our target is the very input image. 
}


\response
{
    Table 1: it would be helpful to highlight best numbers in bold
}
{
    This has been addressed, thanks for pointing it out.
}

\response
{
    Table 1: Why is the FID significantly large for 0 and 180 degrees ? It would be useful to have some comments on this.
}
{
   We copy in the following the answer to R1 who had the same doubt.\\
   
    Front and rear views are less common in the \pascal dataset, which makes predictions around those angles particularly challenging.
    In this case our method often operates into an almost complete absence of prior information, as lateral planes will likely have been dropped during the transformation (e.g. when going from left side view to front view the side is not visible anymore in the destination view). This results in a texture-less shape inferred from the 2.5D sketch and a lower \fid.
    
    Also learning-based approaches like VON or TVSN fail more frequently for those viewpoint. However, we observed that the most common failure mode is the generation of a blob-like shape filled with textures from the source image. Even though is extremely unrealistic for the human eye it's rewarded by the \fid as it preserves textures.
}

\response
{
    The experiments are conducted on a relatively low resolution of 128x128. Is there a reason for that ?
}
{
    The choice of the resolution (128x128) allows both for fast training times and it is shared by the majority of our competitors. Hence, it was a natural choice to allow for a fair comparison with the current state-of-the-art. Additionally, a noticeable share of Pascal+ crops (especially for the vehicle subset) has itself a very low resolution.
}

\response
{
    The introduction mentions using the symmetry constraints but it is not clear where is that used in the method. is it only applied through the appearance prior? 
}
{
    For the car subset in particular, the symmetry constraint is used between the two side views. If we start from a left side view and our target has the car's right side visible, we can flip the source left one and paste it into the correct channel in the input tensor. This allows our method to still access prior information in situations where it wouldn't have any plane information available.
}


==> tables/fid.tex <==
\begin{table}
\begin{center}
\begin{tabular}{lc}
    \toprule
    & Car\\
    \midrule
    Pix2pix~\cite{isola2017image}      &  00.0 \\
    CycleGAN~\cite{zhu2017unpaired}    &  00.0 \\
    \vunet~\cite{esser2018variational} &  00.0 \\
    \von~\cite{zhu2018visual}           &  00.0 \\
    \vonfinetuned~\cite{zhu2018visual}           &  00.0 \\
    \textbf{ours}                      &  \textbf{00.0} \\
    \bottomrule
\end{tabular}
\end{center}
\caption{\fids~\cite{heusel2017gans} results. Each row reports the average distance between real and generated images for each method on the left. \plz{Maybe train DCGAN? Since alignment is not required...}}
\label{tab:fid}
\end{table}
